Lovasz Convolutional Networks

Semi-supervised learning on graph structured data has received significant attention with the recent introduction of Graph Convolution Networks (GCN). While traditional methods have focused on optimizing a loss augmented with Laplacian regularization framework, GCNs perform an implicit Laplacian type regularization to capture local graph structure. In this work, we propose Lovasz Convolutional Network (LCNs) which are capable of incorporating global graph properties. LCNs achieve this by utilizing Lovasz's orthonormal embeddings of the nodes. We analyse local and global properties of graphs and demonstrate settings where LCNs tend to work better than GCNs. We validate the proposed method on standard random graph models such as stochastic block models (SBM) and certain community structure based graphs where LCNs outperform GCNs and learn more intuitive embeddings. We also perform extensive binary and multi-class classification experiments on real world datasets to demonstrate LCN's effectiveness. In addition to simple graphs, we also demonstrate the use of LCNs on hyper-graphs by identifying settings where they are expected to work better than GCNs.

==> sections/background.tex <==
\section{Background}
In this section, we describe graph semi-supervised learning and how recent work has used graph convolutions to address it along with the motivation of our proposed solution.


\subsection{Graph-based Semi Supervised Learning (SSL)}
Often we come across cases where obtaining data samples is easy but labels are available for only a small subset of the data, such a paradigm is known as Semi-Supervised Learning(SSL). The objective is to predict labels for the rest of data points. SSL Learning on graphs, \cite{sslintroicml03}, \cite{sslintronips03}, \cite{sslintro06}, \cite{sslintro09} represents tasks where small portion of graph-structured data is labelled. For example, node classification task, where given a graph and labels for some of the vertices, the aim is to classify remaining vertices to these labels. Where labels may have physical meaning like, say people with the same label belong to the same community. Conventionally, the graph structure is used as an explicit regulariser, $\mathcal{L}_{reg}$ along with the SSL loss over the vertex labelled data, $\mathcal{L}_{0}$. The term $\mathcal{L}_{reg}$ act as a link between edge based similarity and vertex similarity, which tries enforce the use of edge similarity to predict vertex similarity. But the regulariser term is not used to diffuse the information from the labelled data.
\begin{equation}\label{eq1}
	\mathcal{L} = \underbrace{\mathcal{L}_{0}}_\text{\small{labeled data}} + \underbrace{\lambda\mathcal{L}_{reg}}_\text{\small{graph data}}
\end{equation}

\subsection{Graph Convolutions for Graph-based SSL} To avoid this explicit regularisation, which assumes connected nodes to be similar in some sense, we use an implicit convolution neural network based regulariser. This gives us a representation of all the nodes, which uses the kernel similarity and labels information to predict labels for rest of the nodes. Recent works such as \cite{dcnn_nips16} and \cite{gcniclr17} encode both the labelled and the graph data using a convolutional type neural network.
This allows the network to be trained on a supervised loss function $\mathcal{L} = \mathcal{L}_{0}$ for all graph nodes.

\subsection{Motivation for Lov{\'a}sz Kernel}
A typically used graph-based regulariser is the graph Laplacian which relies on the prior assumption that connected nodes in the graph are likely to share the same label (the cluster assumption \cite{ca02}).
This assumption might restrict modelling capacity, as graph edges
encode similarity just based on the connectivity properties of the graph, but the similarity of nodes can be represented in terms of other graph properties as well. We propose the use of Lov{\'a}sz kernel as the similarity measure and show superior performance on graph SSL tasks. Lov{\'a}sz orthogonal embeddings have found there Applications to Max-Cut, Clustering, Summarization \cite{NIPS2015_5902} and finding large dense sub-graphs \cite{JMLR:v14:jethava13a}. All these papers have pointed out the effectiveness of Lovasz kernel at capturing global graph structure.

==> sections/problem.tex <==
\section{Graph SSL via Lovasz-GCN: Our approach}
Similarity of vertices can be defined in several ways which can depend highly on the tasks specified. For example, similarity can be defined in terms of colouring properties of the graph. For this purpose, we relax the condition of using the adjacency matrix and propose Lovasz kernel $K$ which captures the global graph structure.

\subsection{Lov{\'a}sz Orthogonal Representation}
\begin{definition}[Lov{\'a}sz Orthonormal Representation]
	Let $G=(V,E)$ in $\mathbb{R}^d$ assigns to each $i \in V$ a non-zero vector $u_i \in \mathbb{R}^d$ such that $u_i^T u_j = 0$ whenever $(i,j)\in \bar{E}$ and $|| u_i||=1 \; \forall i \in V$. 
\end{definition}
\begin{definition}[Lov{\'a}sz Theta Function]
	The smallest angle of a rotational cone (in arbitrary dimension) which contains all vectors in the orthogonal representation of the graph gives rise to the theta-function of the graph.
	\[\vartheta(G) = \min_{(u_i),c} \max_{i \in V} \frac{1}{(c^T u_i)^2}\]
	where minimum is taken over all the orthonormal representations $(u_i:i \in V)$ of $G$ and all unit vectors $c$.
\end{definition}
\begin{theorem}[Lov{\'a}sz Sandwich Theorem]
	For every graph $G$, $\alpha(G) \leq \vartheta(G) \leq \chi(\bar{G})$, where $\alpha(G)$ is size of maximal independent set and $\chi(G)$ is the colouring number of $G$.
\end{theorem}
\begin{definition}[Perfect graphs]
	A graph $G$ is perfect if for all induced sub-graphs $H$ of $G$, clique number is equal to chromatic number i.e. $\omega(H) = \chi(H)$
\end{definition}
\begin{theorem}
	If $G$ is perfect then, $\alpha(G) = \vartheta(G) = \chi(\bar{G})$
\end{theorem}
\subsection{Lov{\'a}sz Orthogonal Embedding and Kernel}
Lov{\'a}sz theta function can also be represented in terms of a semi-definite program as follows:
\begin{equation*}
	\begin{aligned}
		& {\text{minimize}}
		& & t 
		& \text{subject to}
		& & Y \succeq 0, \;Y_{ij} = -1, \; \forall(i,j) \in \bar{E}, \; Y_{ii} = t-1
	\end{aligned}
\end{equation*}
As $Y$ is a positive semi-definite, so it can be written as a Gram Matrix, i.e, there are vectors $x_i \in \mathbb{R}^n$ such that
\[ Y = x_i^T x_j = \begin{cases} 
-1 & \text{if }(i,j) \in \bar{E}\\
t-1 & \text{if }i=j
\end{cases}
\]
(no condition if $(i,j) \in E$), Let $c$ be a vector orthogonal to all the $x_i$, increase dimension if necessary, and set $u_i = \frac{(c+x_i)}{\sqrt{t}}$. The $u_i^Tu_i = 1$ and $u_i^Tu_j=0 \; \forall (i,j) \in \bar{E}$. Hence $(u_i)$ is an orthonormal representation and the Lov{\'a}sz kernel is a matrix $K$ such that $K_{ij}=u_i^T u_j$. The LS labelling kernel can also be used instead of the Lovasz kernel.

\subsection{GCNs for graph-based semi-supervised node classification}
\label{GSSL}
The GCN is conditioned on both the Lovasz kernel $K$ and the data matrix $X$ (input features). The forward model for a simple two-layer GCN takes the following simple form as in \cite{gcniclr17}:
\begin{equation}
	\label{gcn}
	Z = f_{GCN}(X,K) = \text{softmax}\Big(K\ \text{ReLU}\big(K X\Theta^{(0)}\big)\Theta^{(1)}\Big) 
\end{equation}
where diagonals of $K$ should be $1$ and $\Theta^{(0)}\in\mathbb{R}^{p\times h}$ is an input-to-hidden weight matrix for a hidden layer with $h$ hidden units and $\Theta^{(1)}\in\mathbb{R}^{h\times q}$ is a  hidden-to-output weight matrix.
The softmax activation function defined as $\text{softmax}(x_i) = \frac{\text{exp}(x_i)}{\sum_i\text{exp}(x_i)}$ is applied row-wise.

\textbf{Training} For semi-supervised multi-class classification with $q$ classes, we then evaluate the cross-entropy error over all the set of labelled examples, $\mathcal{V}_L$:
\begin{equation}
	\label{sslgcnloss}
	\mathcal{L} = -\sum_{i\in \mathcal{V}_L}\sum_{j=1}^q Y_{ij}\ln Z_{ij} 
\end{equation}
The weights of the graph convolutional network, viz. $\Theta^{(0)}$ and $\Theta^{(1)}$ are trained using gradient descent. 
Using efficient sparse-dense matrix multiplications for computing, the computational complexity of evaluating Eq. ~\ref{gcn} is $O(|\mathcal{E}|phq)$ which is linear in the number of graph edges.

==> sections/related_work.tex <==
\section{Related Work}

\begin{itemize}
	\item Diffusion CNN
	\item Fast localised spectral filtering
	\item Kipf SSL 
	\item the emerging field of signal processing
	\item Geometric deep learning going beyond euclidean space.
	\item Lovasz theta finding dense sub-graphs
	\item lovasz application to clustering, max-cut, etc.
	\item A convex quadratic characterisation of lovasz theta function
	\item weighted theta function.
	\item Geometric representation of graphs.
	\item 
\end{itemize}

Semi-supervised learning on graph 
In this section, we define spectral and spatial GCN and provide a different interpretation of these networks.
\textbf{Spectral GCN via graph Fourier Transform: } 
Given an undirected connected graph, $\mathcal{G} = (\mathcal{V}, \mathcal{E})$, where $\mathcal{V}$ is finite set of $|\mathcal{V}|=n$ vertices, $\mathcal{E}$ is a set of edges. $A$ represents the adjacency matrix encoding the connection between any two vertices A signal $f:\mathcal{V} \rightarrow \mathbb{R}$ defined on the nodes of the graph can be regarded as a vector $x \in \mathbb{R}^n$ where $x_i$ is the value at $i^{th}$ node. The normalised laplacian is $\mathcal{L}=I_n-D^{-\frac{1}{2}}AD^{-\frac{1}{2}}$, where $I_n$ is the identity and $D=diag(\sum_{j}A_{ij})$ is the diagonal degree matrix. $\mathcal{L}$ is real symmetric positive semi-definite matrix, hence it has a complete set of eigenvectors $\{u_l\}_{l=0}^{n-1} \in \mathbb{R}^n$ which acts as Fourier basis and the corresponding set of eigenvalue $\{\lambda_l\}_{l=0}^{n-1}$, identified as the frequencies of the graph. The laplacian is diagonalised by the Fourier basis $U = [u_0,\ldots,u_{l-1}] \in \mathbb{R}^{n \times n}$ such that $\mathcal{L}=U \Lambda U^T$ where $\Lambda = diag([\lambda_0,\ldots,\lambda_{n-1}]) \in \mathbb{R}^{n \times n}$. The graph Fourier transform of a signal $f\in\mathbb{R}^n$ is then defined as $\hat{f}=U^Tf \in \mathbb{R}^n$ and it's inverse as $f = U\hat{f}$. Given this machinery we can formulate fundamental signal processing operation such as filtering, convolution among others as in \cite{DBLP:journals/corr/DefferrardBV16} and \cite{DBLP:journals/corr/abs-1211-0053}.


\textbf{Spectral Filtering and Convolutions on Graphs:} Convolutions are defined as $x *_g y = U((U^T x)\odot (U^T y)$, where $\odot$ is the element-wise product, this definition is designed to respect the convolution theorem.
A signal $x$ filtered by a filter $g_\theta$ is defined as 
$y = g_\theta (\mathcal{L})f = g_\theta(U\Lambda U^T)f = U g_\theta(\Lambda)U^T f $. If $g_\theta = diag(\theta)$ then the filter is non parametric.\\

\textbf{Spatial GCN: } Graph convolution can also be defined in the spatial domain i.e the vertex domain as in \cite{gcniclr17}. The idea is that the embedding of a node should be affected by the embeddings of it's neighbours as they are similar in some sense. The feature update for each GCN layer can be written as,
\[ f_i^{(l+1)} = \sigma( w_{i}f_i^{(l)} + \sum_{j \in \mathcal{N}(i)} w_{j} f_j^{(l)} )\]
So applying l-layers of GCN diffuses information from all the vertices in the k-hop neighbourhood of $i$. In matrix notation, it can be written as \[F^{(l+1)} = \sigma(\tilde{A} F^{(l)}W^{(l)})\] where $\tilde{A} = A + I$, $A$ is the adjacency, $\sigma$ denotes the activation function, $F^{(l)}$ is the node representation obtained after the $l^{th}$ layer and $F^{(0)}=X$. We added $I$ as graph $G$ has no self loops but still we want the embedding of the node to affect itself.\\
\textbf{Interpretation: }In signal processing term we can interpret the equation as follows, Each column in $W$ is a filter which when pre-multiplied with the matrix $F^{(l)}$ returns the filtered signal/feature on the graph. The multiplication with the matrix $\tilde{A}$ combines these filtered signal according to the graph structure to get a new diffused set of signal for the vertices. Usually a normalised version of $\tilde{A}$ is used for faster convergence and stability of the algorithm, like the laplacian $\tilde{\mathcal{L}}$. Laplacian contains information about the similarity of vertices based on the connection properties.
